Secure mmWave Beamforming with Proactive-ISAC Defense Against Beam-Stealing Attacks

Millimeter-wave (mmWave) communication systems face increasing susceptibility to advanced beam-stealing attacks, posing a significant physical layer security threat. This paper introduces a novel framework employing an advanced Deep Reinforcement Learning (DRL) agent for proactive and adaptive defense against these sophisticated attacks. A key innovation is leveraging Integrated Sensing and Communications (ISAC) capabilities for active, intelligent threat assessment. The DRL agent, built on a Proximal Policy Optimization (PPO) algorithm, dynamically controls ISAC probing actions to investigate suspicious activities. We introduce an intensive curriculum learning strategy that guarantees the agent experiences successful detection during training to overcome the complex exploration challenges inherent to such a security-critical task. Consequently, the agent learns a robust and adaptive policy that intelligently balances security and communication performance. Numerical results demonstrate that our framework achieves a mean attacker detection rate of 92.8% while maintaining an average user SINR of over 13 dB.

==> Table/table1.tex <==
\begin{table*}[!t]
\caption{Comprehensive Simulation Configuration and Parameters}
\label{tab:detailed_sim_params}
\renewcommand{\arraystretch}{1.3}
\setlength{\tabcolsep}{4pt}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{4}{|c|}{\textbf{System Configuration Parameters}} \\
\hline
\textbf{Category} & \textbf{Parameter} & \textbf{Value} & \textbf{Notes} \\
\hline
\multirow{9}{*}{\textbf{MIMO}} & Tx Antennas & 4 & \multirow{2}{*}{Fixed 4×4 MIMO setup} \\
\cline{2-3}
 & Rx Antennas & 4 & \\
\cline{2-4}
 & Array Type & ULA & Uniform Linear Array \\
\cline{2-4}
 & Streams & 4 & Equal to antenna count \\
\cline{2-4}
 % & Element Spacing & 0.5\lambda & Half wavelength \\
 & Element Spacing & \(0.5\lambda\) & Half wavelength \\

\cline{2-4}
 & Polarization & Single & Base configuration \\
\cline{2-4}
 & Antenna Gain & 5-15 dBi & Realistic signal modeling \\
\cline{2-4}
 & Pattern & Directional & Custom beam patterns \\
\cline{2-4}
 & Orientation & Az./El. Angles & Random for diversity \\
\hline
\multirow{6}{*}{\textbf{Resource Grid}} & Subcarriers & 64 & Sionna standard \\
\cline{2-4}
 & Spacing & 30 kHz & 5G NR numerology 1 \\
\cline{2-4}
 & OFDM Symbols & 14 & One slot duration \\
\cline{2-4}
 % & Symbol Duration & 71.4 μs & Including cyclic prefix \\

 & Symbol Duration & $71.4\mu\text{s}$ & Including cyclic prefix \\
 
\cline{2-4}
 & Bandwidth & 2 MHz & Matches subcarrier config \\
\cline{2-4}
 & Modulation & QPSK & Adaptive modulation \\
\hline
\multirow{8}{*}{\textbf{Channel Model}} & Type & Rayleigh Block & Supported in Sionna \\
\cline{2-4}
 & Paths & 10 & Multipath simulation \\
\cline{2-4}
 & User Type & Static & Fixed RX devices \\
\cline{2-4}
 & Path Loss & FSPL & Free Space model \\
\cline{2-4}
 & SNR Range & 0-30 dB & Test configuration \\
\cline{2-4}
 % & Delay Spread & 0.1-1 μs & Realistic dispersion \\

 & Delay Spread & $0.1$--$1\,\mu\text{s}$ & Realistic dispersion \\

\cline{2-4}
 & Interference & Co-channel & Fixed patterns \\
\cline{2-4}
 & Height & 1.5m & Fixed antenna height \\
\hline
\multirow{6}{*}{\textbf{Training}} & Architecture & SAC & Deep RL approach \\
\cline{2-4}
 & Dataset Size & \begin{tabular}[t]{@{}l@{}}Train: 1.32M\\Val/Test: 100K each\end{tabular} & Comprehensive split \\
\cline{2-4}
 & Episodes & 100K & Total training runs \\
\cline{2-4}
 & Learning Rates & All 3e-4 & Actor/Critic/Alpha \\
\cline{2-4}
 & Discount Factor & 0.99 & Standard RL config \\
\cline{2-4}
 & Batch Size & 256 & Gradient updates \\
\hline
\multirow{5}{*}{\textbf{Performance}} & BER & < 10\textsuperscript{-5} & At 15 dB SNR \\
\cline{2-4}
 & Throughput & > 95\% & Of theoretical max \\
\cline{2-4}
 & Latency & < 1ms & Per inference \\
\cline{2-4}
 & Spectral Eff. & 4-8 bits/s/Hz & Static environment \\
\cline{2-4}
 & SINR & > 15 dB & Quality threshold \\
\hline
\multirow{4}{*}{\textbf{Dataset}} & Size & 1.32M samples & Balanced complexity \\
\cline{2-4}
 & Noise Floor & -174 dBm/Hz & Thermal noise base \\
\cline{2-4}
 & Random Seed & Fixed & Reproducible results \\
\cline{2-4}
 & Configuration & Static & Fixed parameters \\
\hline
\end{tabular}
\end{table*}

==> Table/table2.tex <==
\begin{table}[!t]
\centering
\renewcommand{\arraystretch}{1.15}
\scriptsize
\setlength{\tabcolsep}{3.5pt}
\caption{Comparison between Causal Inference and XAI Approaches}
\label{tab:causal-vs-xai}
\begin{tabular}{@{}p{0.85cm}p{2.2cm}p{2.2cm}@{}}
\toprule
\textbf{Feature} & \textbf{Causal Inference} & \textbf{XAI} \\
\midrule

\textbf{Goal} & 
Find true cause of beam switches & 
Explain AI beam selection \\
\midrule

\textbf{Key Q.} & 
``Would switch occur without obstacle?'' & 
``Why this beam vs. others?'' \\
\midrule

\textbf{Focus} & 
Avoid unnecessary switching & 
Increase trust \& trans\-parency \\
\midrule

\textbf{Method} & 
SCM, DoWhy, Count\-erfactual & 
SHAP, LIME, Feature Importance \\
\midrule

\textbf{Data} & 
Historical data needed & 
Works with live decisions \\
\midrule

\textbf{Output} & 
Optimize switching policy & 
Explain beam\-forming decisions \\
\midrule

\textbf{6G Use} & 
Self-learning adapt\-ation & 
Human-in-loop \& transparency \\
\bottomrule
\end{tabular}
\vspace{-3pt}
\end{table}
